LinKS: Discovering galaxy-scale strong lenses in the Kilo-Degree Survey using Convolutional Neural Networks

We present a new sample of galaxy-scale strong gravitational-lens candidates, selected from 904 square degrees of Data Release 4 of the Kilo-Degree Survey (KiDS), i.e., the "Lenses in the Kilo-Degree Survey" (LinKS) sample. We apply two Convolutional Neural Networks (ConvNets) to $\sim88\,000$ colour-magnitude selected luminous red galaxies yielding a list of 3500 strong-lens candidates. This list is further down-selected via human inspection. The resulting LinKS sample is composed of 1983 rank-ordered targets classified as "potential lens candidates" by at least one inspector. Of these, a high-grade subsample of 89 targets is identified with potential strong lenses by all inspectors. Additionally, we present a collection of another 200 strong lens candidates discovered serendipitously from various previous ConvNet runs. A straightforward application of our procedure to future Euclid or LSST data can select a sample of $\sim3000$ lens candidates with less than 10 per cent expected false positives and requiring minimal human intervention.

==> table_candidates.tex <==
RA & DEC & score & $p_1$ & $p_3$ & $g$ & $r$ & $i$ & \sigs\ [km/s] &\\
\hline
805 & 159.78072 & -2.27497 & 70 & 1.0 & 0.999 & 18.6585178375 & 17.2346248627 & 16.8726062775 &  &                                        &             \\
1588 & 333.41257 & -33.19898 & 70 & 0.999 & 0.999 & 18.3788967133 & 16.9627742767 & 16.577835083 &  & 0.25                                &             \\
2075 & 338.65674 & -32.36358 & 70 & 0.957 &  & 16.8039855957 & 15.7488565445 & 15.3261241913 &  & 0.170000001788                          &             \\
2854 & 46.66543 & -27.60745 & 70 & 1.0 & 1.0 & 21.8361358643 & 19.0291156769 & 18.1261043549 &  &                                         &             \\
51 & 178.21776 & 0.79257 & 64 & 0.989 & 0.9 & 21.2585983276 & 19.7089557648 & 18.9489192963 &  & 0.469999998808                           &             \\
2251 & 131.33397 & -0.91563 & 64 & 0.887 & 0.901 & 20.6122913361 & 18.8769512177 & 18.2345218658 & 0.4027400016784668 & 0.449999988079    &             \\
2729 & 203.7478 & 0.27151 & 64 & 1.0 & 1.0 & 20.8616695404 & 19.2739715576 & 18.5046958923 & 0.48362666 &                                 & $259 \pm 31 $   \\
3096 & 357.76907 & -32.88947 & 64 &  & 0.937 & 19.1726703644 & 17.7389774323 & 17.227848053 & 0.28742000460624695 & 0.270000010729        &             \\
248 & 176.18675 & 0.22968 & 58 & 0.95 & 0.96 & 21.473651886 & 19.4317531586 & 18.7027721405 & 0.9411699 &                                 & $145 \pm 179$   \\
329 & 200.23593 & 1.66408 & 58 &  & 0.929 & 19.9740905762 & 18.4114208221 & 17.9091396332 & 0.2970464 &                                   & $214 \pm 16 $   \\
704 & 221.51454 & -0.67129 & 58 & 0.937 & 0.959 & 19.3728809357 & 17.7181777954 & 17.2814083099 & 0.287607 & 0.389999985695               & $270 \pm 21 $   \\
738 & 23.51542 & -30.54075 & 58 &  & 0.948 & 20.752248764 & 19.3524303436 & 18.6359596252 & 0.31766000390052795 &                         &             \\
1038 & 215.64755 & -2.64925 & 58 & 0.999 & 1.0 & 20.7602005005 & 18.9282455444 & 18.4033794403 & 0.3913443 & 0.519999980927               & $239 \pm 26 $   \\
1078 & 356.83185 & -33.50623 & 58 & 0.987 & 0.953 & 20.3965091705 & 18.7896709442 & 18.1487426758 & 0.46838000416755676 & 0.490000009537  &             \\
1642 & 175.87355 & -1.74164 & 58 & 0.999 &  & 16.6464271545 & 15.6369628906 & 15.2545642853 & 0.106046475 & 0.15000000596                 & $262 \pm 5  $   \\
2058 & 183.07338 & 1.88558 & 58 & 0.907 &  & 20.3390769958 & 18.4420871735 & 17.9114837646 & 0.38137618 & 0.449999988079                  & $274 \pm 23 $   \\
3157 & 349.1903 & -29.3954 & 58 & 0.992 & 0.999 & 21.8603515625 & 19.8121738434 & 18.95271492 &  &                                        &             \\
2558 & 133.69397 & -1.36032 & 54 & 1.0 & 0.999 & 19.7875995636 & 17.9025325775 & 17.28399086 & 0.35561999678611755 & 0.419999986887       &             \\
3154 & 204.68665 & -1.15136 & 52 & 1.0 & 1.0 & 20.6736412048 & 18.8600749969 & 18.3516349792 & 0.4238302 &                                & $279 \pm 38 $   \\
3261 & 230.63187 & -0.75082 & 52 & 0.911 & 0.908 & 21.439289093 & 19.336889267 & 18.6847019196 & 0.49764422 &                             & $293 \pm 37 $   \\
726 & 31.61951 & -33.79683 & 48 & 0.989 & 0.976 & 20.3255062103 & 18.7127552032 & 18.1928730011 &  &                                      &             \\
1282 & 335.37155 & -34.94455 & 48 & 0.918 & 0.931 & 20.0539627075 & 18.6515884399 & 18.1197566986 &  &                                    &             \\
2318 & 21.81908 & -33.36483 & 48 & 0.998 &  & 16.970905304 & 15.833278656 & 15.4200429916 &  &                                            &             \\
352 & 34.46518 & -31.0478 & 46 & 0.99 &  & 19.3848457336 & 17.8505916595 & 17.3480224609 &  & 0.270000010729                              &             \\
1351 & 352.77313 & -33.97491 & 46 & 0.995 & 0.987 & 18.5345726013 & 17.284040451 & 16.8122081757 &  & 0.259999990463                      &             \\
1276 & 238.00044 & -1.78534 & 44 & 0.991 &  & 18.2194004059 & 16.8446979523 & 16.3071422577 &  &                                          &             \\
1231 & 188.59088 & -0.1572 & 42 & 0.994 & 1.0 & 21.0311641693 & 19.290851593 & 18.7963790894 &  &                                         &             \\
1258 & 216.7776 & 0.7208 & 42 &  & 0.94 & 19.5233039856 & 18.0792293549 & 17.5073432922 & 0.29516897 & 0.330000013113                     & $228 \pm 19 $   \\
1938 & 129.35904 & 1.94427 & 42 & 0.903 & 0.992 & 20.4824829102 & 18.9138870239 & 18.3629837036 & 0.3957978 & 0.330000013113              & $215 \pm 25 $   \\
2187 & 183.60019 & -0.53509 & 42 & 0.968 & 0.997 & 19.0999698639 & 17.793170929 & 17.2532482147 & 0.24790788 & 0.34999999404              & $239 \pm 37 $   \\
2277 & 198.8718 & 1.53991 & 42 &  & 0.962 & 21.6388931274 & 19.5573863983 & 18.8662624359 &  &                                            &             \\
3302 & 20.44706 & -28.75272 & 42 &  & 0.814 & 21.4181346893 & 19.2353458405 & 18.5917186737 & 0.448419988155365 &                         &             \\
231 & 37.77798 & -32.97901 & 40 & 0.997 & 0.999 & 21.7951221466 & 19.9222984314 & 19.2663249969 & 0.5146200060844421 &                    &             \\
1012 & 46.41708 & -29.5711 & 40 & 0.908 & 0.971 & 20.5694236755 & 18.7429008484 & 18.2798576355 &  &                                      &             \\
1849 & 204.2834 & 1.2177 & 38 &  & 0.953 & 19.5296840668 & 17.6767063141 & 17.2018146515 & 0.32722294 &                                   & $289 \pm 21 $   \\
3098 & 181.19672 & -2.72009 & 38 & 0.962 &  & 14.4921274185 & 13.7894773483 & 13.4792480469 & 0.01960516 & 0.119999997318                 & $110 \pm 4  $   \\
105 & 215.70692 & -0.55323 & 36 &  & 0.975 & 21.2148952484 & 19.3766384125 & 18.6798782349 & 0.4530718 & 0.509999990463                   & $258 \pm 29 $   \\
326 & 186.20958 & -0.70414 & 36 & 0.998 & 0.989 & 20.2567329407 & 18.3892669678 & 17.7710723877 & 0.40306014 & 0.460000008345             & $319 \pm 35 $   \\
365 & 141.1433 & -1.90478 & 36 & 0.849 &  & 20.0629253387 & 18.4802913666 & 17.7169799805 &  &                                            &             \\
534 & 185.64714 & -2.42117 & 36 & 0.99 &  & 19.9099292755 & 18.6159915924 & 17.994852066 & 0.2555899918079376 & 0.300000011921            &             \\
1093 & 199.99738 & 2.11804 & 36 & 0.851 &  & 18.9425773621 & 17.5716609955 & 17.186170578 & 0.21544546 &                                  & $240 \pm 12 $   \\
2199 & 350.62283 & -30.6434 & 36 & 0.983 & 0.905 & 19.5693130493 & 18.1857452393 & 17.7195243835 &  & 0.310000002384                      &             \\
2313 & 221.67886 & -3.85043 & 36 & 0.954 & 0.891 & 21.06366539 & 19.438129425 & 18.8108329773 &  &                                        &             \\
2769 & 186.161 & -0.69799 & 36 & 0.997 & 1.0 & 20.2990455627 & 18.7070102692 & 18.1189975739 &  & 0.509999990463                          &             \\
3351 & 37.39024 & -30.83811 & 36 & 0.93 & 0.999 & 21.6926212311 & 19.6805782318 & 18.9454269409 & 0.5119699835777283 &                    &             \\
1364 & 31.27489 & -33.29631 & 34 &  & 0.908 & 20.8331298828 & 18.9517993927 & 18.2593154907 &  &                                          &             \\
2161 & 345.1022 & -35.209 & 34 &  & 0.998 & 20.6379814148 & 18.8822898865 & 18.3212566376 & 0.31404000520706177 &                         &             \\
2602 & 10.94209 & -30.82482 & 34 & 0.819 & 0.967 & 20.3126087189 & 18.7663593292 & 18.2167472839 &  &                                     &             \\
2632 & 10.5192 & -32.53961 & 34 & 0.94 & 0.98 & 20.8520755768 & 19.1436252594 & 18.6622409821 &  &                                        &             \\
315 & 220.63545 & 0.29188 & 32 &  & 0.8 & 18.6425991058 & 17.4808750153 & 17.0424022675 & 0.20748243 & 0.300000011921                     & $171 \pm 12 $   \\
430 & 35.6577 & -32.15816 & 32 & 0.984 & 0.835 & 19.2993373871 & 17.799577713 & 17.3397483826 &  &                                        &             \\
817 & 180.41615 & -0.20731 & 32 & 0.988 & 0.929 & 19.19099617 & 17.8184585571 & 17.3694992065 & 0.24944999814033508 &                     &             \\
844 & 16.67529 & -34.40028 & 32 & 0.983 & 0.993 & 19.7794380188 & 18.3921737671 & 17.8524475098 &  &                                      &             \\
891 & 331.5931 & -33.04589 & 32 & 0.891 & 0.883 & 21.3152713776 & 19.6097145081 & 18.9589290619 &  & 0.449999988079                       &             \\
909 & 185.67223 & 2.09977 & 32 & 1.0 &  & 18.5443668365 & 17.0142650604 & 16.472076416 & 0.22866239 & 0.289999991655                      & $304 \pm 17 $   \\
1125 & 22.6289 & -30.45799 & 32 & 0.968 & 0.983 & 20.0466804504 & 18.3921165466 & 17.7940216064 &  &                                      &             \\
3142 & 232.0035 & 0.67562 & 32 & 0.889 & 0.983 & 20.6127166748 & 18.9310874939 & 18.4611606598 & 0.56022656 & 0.34999999404               & $244 \pm 41 $   \\
259 & 331.6506 & -32.71608 & 30 & 0.812 & 0.975 & 19.8937358856 & 18.5330677032 & 17.96824646 &  & 0.330000013113                         &             \\
496 & 50.58249 & -34.41571 & 30 & 0.844 & 0.882 & 20.5797328949 & 18.6807804108 & 17.8817157745 &  & 0.419999986887                       &             \\
508 & 155.5362 & -0.4215 & 30 & 0.995 & 0.91 & 20.2592773438 & 18.3030281067 & 17.6249141693 & 0.39399034 &                               & $277 \pm 29 $   \\
897 & 40.00337 & -34.30345 & 30 & 0.974 &  & 18.8722267151 & 17.6825561523 & 17.2172966003 &  & 0.25                                      &             \\
1148 & 357.74005 & -34.41555 & 30 & 0.998 & 0.958 & 20.4392662048 & 18.6202888489 & 17.9821205139 & 0.3626599907875061 &                  &             \\
1242 & 47.19172 & -29.05714 & 30 & 0.918 &  & 20.3461608887 & 18.6386947632 & 18.2055740356 & 0.3653300106525421 &                        &             \\
1349 & 345.10303 & -35.20935 & 30 & 0.996 & 1.0 & 21.5433311462 & 19.6347904205 & 18.8861618042 &  &                                      &             \\
1426 & 176.58809 & -1.68118 & 30 & 0.923 & 0.908 & 21.2589626312 & 19.3960018158 & 18.7530269623 &  &                                     &             \\
1592 & 226.11102 & -1.70997 & 30 &  & 0.915 & 18.9153709412 & 17.8281116486 & 17.2999420166 & 0.13895495 &                                & $203 \pm 17 $   \\
2280 & 334.00406 & -27.76236 & 30 &  & 0.949 & 20.6813850403 & 18.9193935394 & 18.4786987305 &  &                                         &             \\
2367 & 48.84465 & -32.04128 & 30 &  & 0.957 & 20.4664058685 & 18.9182567596 & 18.274848938 &  & 0.319999992847                            &             \\
2369 & 178.83655 & 0.88457 & 30 &  & 0.966 & 19.9655857086 & 18.3859958649 & 17.8893756866 & 0.28277037 & 0.310000002384                  & $213 \pm 20 $   \\
2660 & 132.98734 & 1.50468 & 30 & 0.99 & 0.989 & 19.9228401184 & 18.3406105042 & 17.7758197784 & 0.32721034 & 0.340000003576              & $211 \pm 21 $   \\
2754 & 21.69769 & -28.80421 & 30 & 0.981 & 0.958 & 19.3360958099 & 17.8975734711 & 17.4903736115 & 0.2849000096321106 &                   &             \\
2967 & 130.54643 & 1.64325 & 30 & 1.0 & 1.0 & 20.1705551147 & 18.7217082977 & 18.1502399445 & 0.721589982509613 & 0.479999989271          &             \\
3399 & 205.44713 & -1.94214 & 30 & 0.842 &  & 20.0247745514 & 18.2798118591 & 17.7355613708 & 0.29054025 &                                & $237 \pm 22 $   \\
52 & 205.24345 & -1.85431 & 28 &  & 0.944 & 21.8836269379 & 19.5238208771 & 18.7537002563 & 0.35888842 &                                  & $365 \pm 49 $   \\
562 & 168.98329 & -2.86798 & 28 & 1.0 &  & 19.6701374054 & 17.7650966644 & 17.27576828 & 0.37143046 &                                     & $346 \pm 16 $   \\
1577 & 332.119 & -28.6189 & 28 &  & 0.883 & 20.3884449005 & 18.8394565582 & 18.1379623413 &  &                                            &             \\
1787 & 343.50052 & -34.78101 & 28 & 0.819 & 0.894 & 20.7028503418 & 18.990190506 & 18.4296379089 &  &                                     &             \\
1822 & 183.06471 & 1.91352 & 28 & 0.892 & 0.99 & 20.5038700104 & 18.8956127167 & 18.29479599 & 0.40036175 & 0.430000007153                & $296 \pm 31 $   \\
2322 & 172.90053 & -1.81063 & 28 &  & 0.833 & 19.404510498 & 18.1708316803 & 17.6531009674 &  &                                           &             \\
2379 & 234.30153 & 1.47136 & 28 & 0.94 &  & 18.6511230469 & 17.3996524811 & 16.7574615479 & 0.21360546 &                                  & $225 \pm 14 $   \\
2423 & 207.17921 & -1.94567 & 28 &  & 0.865 & 20.6660175323 & 18.9261341095 & 18.3469791412 & 0.3232828 &                                 & $214 \pm 30 $   \\
2463 & 348.3276 & -29.05727 & 28 & 0.935 &  & 18.8390674591 & 17.4938793182 & 17.1138496399 &  &                                          &             \\
2553 & 179.73003 & -2.51895 & 28 & 0.909 &  & 18.6346302032 & 17.5408096313 & 17.0706100464 & 0.14348218 & 0.170000001788                 & $180 \pm 13 $   \\
2664 & 214.82709 & -0.42031 & 28 & 1.0 & 0.918 & 20.1797008514 & 18.6766052246 & 18.1366081238 & 0.26510000228881836 & 0.340000003576     &             \\
2669 & 140.35284 & -0.97414 & 28 &  & 0.858 & 20.3687286377 & 18.577009201 & 18.0274085999 & 0.3221299946308136 & 0.419999986887          &             \\
2730 & 214.36708 & 1.99311 & 28 & 0.999 & 1.0 & 20.7216262817 & 19.1695022583 & 18.4675006866 & 0.4009086 & 0.430000007153                & $230 \pm 26 $   \\
3222 & 34.10406 & -33.40128 & 28 & 0.905 & 0.878 & 20.7219161987 & 18.9540996552 & 18.3306064606 & 0.39983001351356506 &                  &             \\
3357 & 174.8049 & -0.00257 & 28 & 0.979 & 0.822 & 21.0122909546 & 19.0854187012 & 18.5578098297 & 0.26363998651504517 &                   &             \\
3362 & 170.72163 & -0.03635 & 28 & 0.816 &  & 21.9029369354 & 19.8702945709 & 19.3272647858 & 0.42560983 &                                & $316 \pm 57 $   \\
81 & 231.60757 & 1.95895 & 26 &  & 0.907 & 19.5409679413 & 17.636510849 & 17.0559368134 & 0.30576035 &                                    & $331 \pm 31 $   \\
492 & 0.79235 & -31.87919 & 26 & 0.856 & 0.836 & 20.9472694397 & 19.36095047 & 18.6713848114 &  & 0.469999998808                          &             \\
741 & 0.30467 & -33.36632 & 26 & 0.988 & 0.979 & 19.6846179962 & 18.2938175201 & 17.7178726196 & 0.2720299959182739 & 0.340000003576      &             \\
863 & 40.87669 & -33.67311 & 26 & 0.911 &  & 19.3854103088 & 17.9879055023 & 17.6133975983 &  &                                           &             \\
1064 & 220.38748 & -3.83125 & 26 &  & 0.862 & 19.6918487549 & 18.3529586792 & 17.8442497253 &  &                                          &             \\
1180 & 185.1191 & -1.5125 & 26 & 0.901 & 0.911 & 20.349445343 & 18.7697410583 & 18.2789440155 & 0.2819199860095978 & 0.310000002384       &             \\
1239 & 13.91815 & -30.48673 & 26 &  & 0.837 & 20.4191989899 & 18.8724899292 & 18.206911087 &  &                                           &             \\
1690 & 218.5273 & -0.4848 & 26 &  & 0.888 & 21.0014152527 & 19.2069816589 & 18.6583442688 & 0.33842000365257263 &                         &             \\
1741 & 220.62912 & -0.39809 & 26 & 0.993 & 0.966 & 20.3856086731 & 18.7428531647 & 18.1421318054 & 0.37030175 & 0.449999988079            & $332 \pm 46 $   \\
1851 & 226.08905 & -0.06611 & 26 & 0.993 & 0.999 & 21.0198020935 & 19.3714160919 & 18.8080043793 &  &                                     &             \\
1906 & 129.23265 & -1.57512 & 26 & 0.929 &  & 20.2547416687 & 18.470495224 & 17.8822898865 & 0.3651899993419647 & 0.469999998808          &             \\
1933 & 135.88864 & -0.97487 & 26 &  & 0.883 & 21.0934677124 & 19.1200904846 & 18.5727043152 & 0.4059000015258789 & 0.490000009537         &             \\
2214 & 43.71149 & -31.02942 & 26 & 0.997 &  & 18.5099506378 & 17.0044384003 & 16.4995727539 & 0.29986000061035156 & 0.289999991655        &             \\
2264 & 164.30399 & -1.9052 & 26 & 0.965 & 0.976 & 20.1615352631 & 18.5245704651 & 17.9768600464 & 0.3428392 &                             & $231 \pm 19 $   \\
2382 & 3.8494 & -33.82425 & 26 & 0.809 &  & 19.2223854065 & 17.9140262604 & 17.5077495575 &  & 0.209999993443                             &             \\
2398 & 54.02407 & -33.2057 & 26 & 0.894 &  & 20.684715271 & 19.1197681427 & 18.4888763428 &  &                                            &             \\
2447 & 186.07858 & -1.83749 & 26 & 0.878 & 0.96 & 21.2986850739 & 19.5461597443 & 18.834810257 &  & 0.560000002384                        &             \\
2902 & 13.5148 & -28.40404 & 26 & 0.948 &  & 20.5006198883 & 18.9046993256 & 18.3780708313 & 0.29210999608039856 &                        &             \\
2922 & 182.40587 & -2.63013 & 26 & 0.943 & 0.968 & 20.4830532074 & 19.0223331451 & 18.3909263611 & 0.34158000349998474 & 0.419999986887   &             \\
3102 & 213.5874 & -1.61279 & 26 & 0.803 &  & 21.8543834686 & 19.9159927368 & 19.1857204437 & 0.5114539 &                                  & $310 \pm 31 $   \\
3347 & 227.01643 & -0.89479 & 26 & 0.95 & 0.83 & 21.4238033295 & 19.5079612732 & 18.7009277344 & 0.45198733 &                             & $286 \pm 48 $    \\

